New Aspects of Analyzing Amyloid Fibrils

This is a summary of mathematical tools we used in research of analyzing the structure of proteins with amyloid form \cite{xi2024Top}. We defined several geometry indicators on the discrete curve namely the hop distance, the discrete curvature and the discrete torsion. Then, we used these indicators to analyze the structure of amyloid fibrils by regarding its peptide chains as discrete curves in $\Rds^3$. We gave examples to show that these indicators give novel insights in the characterization analysis of the structure of amyloid fibrils, for example the discrete torsion can detect the hydrogen bonds interactions between layers of amyloid fibril. {Moreover,} the topological tool performs better than the root mean square deviation (RMSD) in quantifying the difference of the structure of amyloid fibrils, etc.

==> contents/intro-tor.tex <==
Many topics in applied geometry like computer graphics and computer vision has close connection with discrete geometry especially the discrete curves and discrete surfaces.
For example the tasks like analysis of geometric data, its reconstruction, and further its manipulation and simulation.
Approximations of 3D-geometric notions play a crucial part in creating algorithms that can handle such tasks.
Similarly as the smooth realm where the curvature and torsion play important rolls in parametrizing a smooth curve or surface, the estimation of curvatures and torsions of curves and surfaces is also important in applied geometry.
%A good understanding of estimating curvatures of curves often serves as an important first step for estimating curvatures of surfaces.

We mention two ways of parametrizing a discrete curve. The first which we call it the (truncated) Hop distance between two discrete curves is defined as a matrix composed of the differences of hop distances of diagonal points between two discrete curves. We will show below by example that this simple defined and computed parameter could 

Recall that the curvature of a smooth curve $\gamma$ at a fixed point $p$ which is defined as the inverse of the radius of the osculating circle of $\gamma$ at point $p$. It quantifies the extent of the bending of $\gamma$ at $p$. The torsion of the curve $\gamma$ given by the 'percentage' between the normal bundle of the curve and the projection of the differential of the binormal bundle on the normal bundle. It measures the speed of a smooth curve moves away from it osculating plane.

In the discrete case we apply the ideas and methods from classical differential geometry instead of “simply” discretizing equations or using classical differential calculus. There are several versions of discretized curvature and torsion based on using different starting point of the classical differential geometry like from Frenet-frame \cite{carroll2014survey} and from geometric knot theory \cite{sullivan2008curves}.
In this paper we will introduce a version of discrete curvature and torsion from \cite{muller2021discrete} which is based on the osculating circle of a discrete curve and we will show an example of its application in analysis structures of the proteins.





